Self-supervised Learning: Generative or Contrastive

Deep supervised learning has achieved great success in the last decade. However, its deficiencies of dependence on manual labels and vulnerability to attacks have driven people to explore a better solution. As an alternative, self-supervised learning attracts many researchers for its soaring performance on representation learning in the last several years. Self-supervised representation learning leverages input data itself as supervision and benefits almost all types of downstream tasks. In this survey, we take a look into new self-supervised learning methods for representation in computer vision, natural language processing, and graph learning. We comprehensively review the existing empirical methods and summarize them into three main categories according to their objectives: generative, contrastive, and generative-contrastive (adversarial). We further investigate related theoretical analysis work to provide deeper thoughts on how self-supervised learning works. Finally, we briefly discuss open problems and future directions for self-supervised learning. An outline slide for the survey is provided.

==> 2-background.tex <==
\section{Background} \label{section:background}
\subsection{Representation Learning in NLP}
Pre-trained word representations are key components in natural language processing tasks. Word embeddings are to represent words as low-dimensional real-valued vectors. There are two kinds of word embeddings: non-contextual and contextual embeddings. 

Non-contextual Embeddings do not consider the context information of the token; that is, these models only map the token into a distributed embedding space. Thus, for each word $x$ in the vocabulary $V$, embedding will assign it a specific vector $e_x\in R^d$, where $d$ is the dimension of the embedding. These embeddings can not model complex characteristics of word usage and polysemy.

To model both complex characteristics of word usage and polysemy, contextual embedding is proposed. For a text sequence $x_1, x_2, ..., x_N$, $x_n \in V$, the contextual embedding of $x_n$ depends on the whole sequence. 
$$[e_1, e_2, ..., e_N] = f(x_1, x_2, ..., x_N),$$
where $f(\cdot)$ is the embedding function. Since for a certain token $x_i$, the embedding $e_i$ can be different if $x_i$  in difference context, $e_i$ is called contextual embedding. This kind of embedding can distinguish the semantics of words in different contexts. 

Distributed word embeddings represent each word as a dense, real-valued, and low-dimensional vector. The first-generation word embedding is introduced as a neural network language model (NNLM)\cite{bengio2003neural}. For NNLM, most of the complexity derives from the non-linear hidden layer in the model. Mikolov et al. proposed Word2Vec Model\cite{Mikolov2013EfficientEO} \cite{mikolov2013distributed} to learn the word representations efficiently. There are two kinds of implementations: Continuous Bag-of-Words Model (CBOW) and Continuous Skip-gram Model (SG). As a kind of context prediction model, Word2Vec is one of the most popular implementations to generate non-contextual word embeddings for NLP.

In the first-generation word embedding, the same word has the same embedding. Since a word can have multiple senses, therefore, the second-generation word embedding methods are proposed. In this case, each word token has its embedding. These embeddings are also called contextualized word embedding since the embeddings of word tokens depend on its contexts. ELMo (Embeddings from Language Model)\cite{peters2018deep} is an implementation to generate those contextual word embeddings. It is an RNN-based bidirectional language model which learns multiple embeddings for each word token, and decides how to combine those embeddings based on the downstream tasks. ELMo is a feature-based approach, that is, the model is used as a feature extractor to extract word embedding, and send those embeddings to the downstream task model. The parameters of the extractor are fixed, and only the parameters in the backend model can be trained.

Recently, BERT (Bidirectional Encoder Representations from Transformers)\cite{devlin2019bert} brings large improvements on 11 NLP tasks. Different from feature-based approaches like ELMo, BERT is a fine-tuned approach. The model is first pre-trained on a large amount of corpora through self-supervised learning, and then fine-tuned with labeled data. As the name indicates, BERT 
% is an encoder of the transformer, 
uses Transformer as its encoder.
In the training stage, BERT masks some tokens in the sentence, and is then trained to predict the masked words. When using BERT, we first initialize the BERT model with pre-trained weights, and then fine-tune the pre-trained model on downstream tasks.


\subsection{Representation Learning in CV}
\hide{The success of automated computer vision systems often hinges on a large amount of labeled data, which is expensive to acquire and not always available. Researchers have devoted significant effort to systems independent of a large amount of expensive supervision. 

Unsupervised visual representation learning remains a mostly unsolved problem in computer vision research. Among a significant body of recently proposed approaches for unsupervised learning of visual representations, a class of self-supervised techniques achieves superior performance on many challenging benchmarks\cite{Kolesnikov2019RevisitingSV}. Most of the prior work endeavors to improve the performance of self-supervised techniques by proposing new pretext tasks. For example, inspired by unsupervised methods from the natural language processing domain which rely on predicting words from their context\cite{Mikolov2013EfficientEO}, Doersch et al. .\cite{doersch2015unsupervised} proposed a practically successful pretext task of predicting the relative location of image patches. Noroozi et al. .\cite{noroozi2016unsupervised} built a model that predicts the permutation of a “jigsaw puzzle” created from the full image. Gidaris et al. \cite{gidaris2018unsupervised} proposed to randomly rotate an image by one of four possible angles and let the model predict that rotation.

Many works have tried to combine multiple pretext tasks. For example, Kim et al. extended the “jigsaw puzzle” task by combining it with colorization and inpainting in \cite{kim2018learning}. Chen et al. \cite{Chen2018SelfSupervisedGV} combined the self-supervised loss from \cite{gidaris2018unsupervised} with the GANs \cite{goodfellow2014generative}objective.  Kolesnikov et al. \cite{Kolesnikov2019RevisitingSV}revealed that neither is the ranking of architectures consistent across different methods, nor is the ranking of methods consistent across architectures, implying that pretext tasks for self-supervised learning should not be considered isolatedly but conjunctively with underlying architectures.}

Computer vision is one of the greatest benefited fields thanks to deep learning. In the past few years, researchers have developed a range of efficient network architectures for supervised tasks. For self-supervised tasks, many of them are also proved to be useful. In this section, we introduce ResNet architecture\cite{he2016deep}, which is the backbone of a large part of the self-supervised techniques for visual representation models. 

%\subsubsection{ResNet architecture}
Since AlexNet\cite{krizhevsky2012imagenet}, CNN architecture is going deeper and deeper. While AlexNet had only five convolutional layers, the VGG network \cite{simonyan2014very} and GoogleNet (also named Inception\_v1) \cite{Szegedy2015GoingDW} had 19 and 22 layers respectively.

Evidence reveals that the network depth is of crucial importance\cite{Szegedy2015GoingDW, simonyan2014very}. Driven by its significance, a question arises: Is learning better networks as easy as stacking more layers? An obstacle to answering this question was the notorious problem of vanishing/exploding gradients \cite{Bengio1994LearningLD}, which hampers convergence from the beginning. This problem, however, has been addressed mainly by normalized initialization \cite{10.5555/645754.668382, Saxe2013ExactST} and intermediate normalization layers \cite{Ioffe2015BatchNA}, which enable networks with tens of layers to start converging for stochastic gradient descent (SGD) with backpropagation\cite{10.1162/neco.1989.1.4.541}.

When deeper networks start to converge, a degradation problem will be exposed: with the increasing network depths, the accuracy soon meets its ceiling (which might be unsurprising) and then degrades rapidly. Unexpectedly, such degradation is not caused by overfitting, and adding more layers to a suitably deep model only leads to higher training error.%, as shown in Fig.  \ref{fig:cv_1} \cite{he2016deep}. 

\hide{
\begin{figure}%[h!]
    \centering
    \includegraphics[width=.48\textwidth]{figs/Background_CV_1.png}
    \caption{Training error (left) and test error (right) on CIFAR-10 with 20-layer and 56-layer “plain” networks. The deeper network has higher training error, and thus test error. \cite{he2016deep}}
    \label{fig:cv_1}
    \vspace{-0.2cm}
\end{figure}
}

Residual neural network (ResNet), proposed by He et al.\cite{he2016deep}, effectively tackles this problem. Instead of asking every few stacked layers to directly learn a desired underlying mapping, the authors design a residual mapping architecture ResNet. The core idea of ResNet is the introduction of “shortcut connections”, which are those skipping over one or more layers.

\hide{
\begin{figure}%[h!]
    \centering
    \includegraphics[width=.48\textwidth]{figs/Background_CV_2.png}
    \caption{Residual learning: a building block.\cite{he2016deep}}
    \label{fig:cv_2}
    \vspace{-0.2cm}
\end{figure}
}

A building block
%shown in Fig. \ref{fig:cv_2} 
 is defined as:

\beq{
y = F (x, \{W_i\}) + x.
}

Suppose $x$ and $y$ are the input and output vectors of the layers. The function $F(x, \{W_i\})$ represents the residual mapping to be learned. For an example cell of ResNet that has two layers, $F = W_2\sigma(W_1x)$ in which $\sigma$ denotes ReLU \cite{Nair2010RectifiedLU} and the biases are omitted for simplifying notations. The operation $F+x$ is performed by a shortcut connection and element-wise addition. 

Because of its compelling results, ResNet has blew people’s minds and quickly become one of the most popular architectures in various computer vision tasks. Since then, ResNet architecture has been drawing extensive attention from researchers, and multiple variants based on ResNet are proposed, including ResNeXt\cite{Xie2017AggregatedRT}, Densely Connected CNN\cite{Huang2017Densely}, and wide residual networks\cite{Zagoruyko2016WideRN}.

\subsection{Representation Learning on Graphs}
As a ubiquitous data structure, graphs are extensively employed in multitudes of fields and become the backbone of many systems. The central problem in machine learning on graphs is to find a way to represent graph structure so that it can be easily utilized by machine learning models~\cite{Hamilton2017RepresentationLO}. To tackle this problem, researchers propose a series of methods for graph representation learning at node level and graph level, which has become a research spotlight recently. 

We first define several basic terminologies.
Generally, a \textit{graph} is defined as $G = (V, E, X)$, where $V$ denotes a set of vertices, $|V|$ denotes the number of vertices in the graph, $E \subseteq (V \times V)$ denotes a set of edges connecting the vertices, and $X \in \mathbb{R}^{|V| \times d}$ is the optional original vertex feature matrix. When input features are unavailable, $X$ is set as orthogonal matrix or initialized with normal distribution, etc., in order to make the input node features less correlated. 

The problem of node representation learning is to learn latent node representations $Z \in \mathbb{R}^{ |V|\times d_z}$, which is also termed as network representation learning, network embedding, etc. There are also some graph-level representation learning problems, which aims to learn an embedding for the whole graph.

\hide{There are many downstream tasks for self-supervised learning on graphs. Node classification, link prediction, clustering are common tasks for node-level representation learning~\cite{Hamilton2017RepresentationLO}. Graph classification, graph generation, graph similarity search are several common tasks for graph-level representation learning. In most cases, node classification is in semi-supervised setting, where only the labels of part of nodes are available, and the goal is to label the full graph. The learned node embeddings can also be used to predict missing edges/links by measuring node proximity, and link prediction is common in social networks~\cite{tang2015line}, recommendation systems~\cite{Berg2017GraphCM} and so on. For graph-level representation learning, the task discussed most in this paper is graph generation. Graph generation is often coupled with specific domains, like molecule graph generation.}

In general, existing network embedding approaches are broadly categorized as (1) factorization-based approaches such as NetMF\cite{Qiu2018NetworkEA, qiu2018network}, GraRep~\cite{Cao2015GraRepLG}, HOPE~\cite{Ou2016AsymmetricTP}, 
(2) shallow embedding approaches
such as DeepWalk~\cite{perozzi2014deepwalk}, LINE~\cite{tang2015line}, HARP~\cite{Chen2018HARPHR}, and (3) neural network approaches\cite{Li2018AdaptiveGC,Cao2016DeepNN}. Recently, graph convolutional network (GCN)\cite{kipf2016semi} and its multiple variants have become the dominant approaches in graph modeling, thanks to the utilization of graph convolution that effectively fuses graph topology and node features. 

However, the majority of advanced graph representation learning methods require external guidance like annotated labels. Many researchers endeavor to propose unsupervised algorithms~\cite{Hamilton2017InductiveRL, Grover2018GraphiteIG,velivckovic2018deep}, which do not rely on any external labels. Self-supervised learning also opens up an opportunity for effective utilization of the abundant unlabeled data~\cite{Sun2020MultiStageSL,Peng2020SelfSupervisedGR}. 
%In this section, we briefly introduce several classic graph representation learning methods in each category.
%, including DeepWalk\cite{perozzi2014deepwalk}, LINE\cite{tang2015line}, and NetMF\cite{Qiu2018NetworkEA}. 
%We also familiarize readers with common benchmark tasks used for evaluating graph representation embeddings, including node classification, link prediction, and graph classification.

\hide{
%\subsubsection{Random Walk Approaches}
\subsubsection{Shallow Embedding Approaches}
%Many recent successful methods learn node embedding based on random walks.
%statistics. 
At the earliest, many network embedding methods employ shallow architectures, which usually only encode direct (first-order) neighbors.
Their key innovation is to optimize the node embeddings so that nodes have similar embeddings if they tend to co-occur on short random walks over the graph~\cite{Hamilton2017RepresentationLO}.

\vpara{DeepWalk} 
DeepWalk~\cite{perozzi2014deepwalk} uses local information obtained from truncated random walks to learn latent representations by treating walks as the equivalent of sentences. The random walk starts in a selected node and then moves to the random neighbor from a current node for a defined number of steps. 

Random walks can be thought of as short sentences and phrases in a particular language.
Therefore, Word2Vec~\cite{xx} technique is employed to learn latent node embeddings by taking walks as sentences. Specifically, DeepWalk uses Skip-Gram to model node sequences, and it uses one node to predict neighboring nodes in the walks. In terms of vertex representation
modeling, this yields the optimization problem:

%The direct analog is to estimate the likelihood of observing vertex $v_i$ given all the previous vertices visited so far in the random walk.

\hide{
\beq{Pr(v_i|(v_1,v_2,...,v_{i-1}))}

The goal of DeepWalk is to learn a latent representation, not only a probability distribution of node co-occurrences, and so authors introduce a mapping function $\Phi{\rm :} v\in V \mapsto \mathbb{R}^{|V|\times d}.$This mapping $\Phi$ represents the latent social representation associated with each vertex $v$ in the graph. The problem then, is to estimate the likelihood:

\beq{Pr(v_i|(\Phi(v_1), \Phi(v_2),...,\Phi(v_{i-1}))).}

However, as the walk length grows, computing this objective function becomes unfeasible. A recent relaxation in language modeling \cite{Mikolov2013EfficientEO,mikolov2013distributed} turns the prediction problem on its head. First, it uses one word to predict the context rather than using the context for words. Second, it considers both sides of a word as context rather than a single side. Third, it removes the ordering constraint by maximizing the probability of the context words without knowing offsets from the given words. In terms of vertex representation modeling, this yields the optimization problem:
}

\beq{
   \minimize\limits_{\Phi} -\log{Pr(\{v_{i-w},...,v_{i-1},v_{i+1},...,v_{i+w}\}|\Phi(v_i))}
}

\noindent where $\Phi(v)$ is the node embedding vector of node $v$. 
By combining both truncated random walks and neural language models, DeepWalk generates node embeddings which preserve graph structures well.
% representations of social networks that are low-dimensional, and exist in a continuous vector space. 
Later then, Grover and Leskovec~\cite{grover2016node2vec} propose node2vec, a network embedding approach with more flexible design of random walks. By introducing two random walk hyperparameters, node2vec is able to generate walks that are more akin to bread-first search (BFS) or depth-first search (DFS).


\vpara{LINE}
Another significantly successful embedding approach is LINE~\cite{tang2015line}, which is efficient on a variety of real-world information networks. LINE combines two encoder-decoder objectives that optimize “first-order” and “second-order” node similarity, respectively.\cite{Hamilton2017RepresentationLO} 

The first-order objective uses a decoder based on the sigmoid function:

\beq{
    \mbox{DEC}(z_i,z_j)=\frac{1}{1+e^{-{z_i}^T{z_j}}}
}

\noindent and an adjacency-based similarity measure.

The second-order encoder-decoder objective is similar but considers two-hop adjacency neighborhoods. Both the first-order and second-order objectives are optimized using loss functions derived from the KL-divergence metric. 


\subsubsection{Factorization-based Methods}
Early methods for learning representations for nodes primarily focused on matrix-factorization approaches, which are directly inspired by classific techniques for dimensionality reduction\cite{Hamilton2017RepresentationLO}.\cite{Qiu2018NetworkEA} proposed a matrix factorization framework NetMF unifying DeepWalk, LINE, PTE, and node2vec.}

\hide{\subsubsection{Benchmark Tasks\cite{Hamilton2017RepresentationLO}}
The most common use cases for graph node embeddings are for node classification, link prediction, and graph classification. Each of these use cases is relevant to many application domains, ranging from computational social science to computational biology.
\vpara{Node Classification}
Node classification is perhaps the most common benchmark task used for evaluating node embeddings. In most cases, a node classification task is a form of semi-supervised learning, where labels are only available for a small proportion of nodes, with the goal being to label the full graph based only on this small initial seed set. 
 
\vpara{Link Prediction}
Node embeddings are also extremely useful as features for link prediction, where the goal is to predict missing edges, or edges that are likely to form in the future\cite{Backstrom2011SupervisedRW}. Link prediction is at the core of recommender systems, and applications of node embeddings reflect this deep connection, including predicting missing friendship links in social networks\cite{tang2015line}and affinities between users and movies\cite{Berg2017GraphCM}. 
 
\vpara{Clustering}
Node embeddings are a powerful tool for clustering related nodes because each node is associated with real-valued vector embedding, it is possible to apply any generic clustering algorithm to the set of learned node embeddings (e.g., k-means or DB-scan\cite{Ester1996ADA}).
}

%\begin{figure*}%[h!]
%    \centering
%    \includegraphics[height=24cm]{figs/Self-supervised.png}
%    \caption{Overview of recent self-supervised representation learning.}
%    \label{fig:ssl}
%    \vspace{-0.2cm}
%\end{figure*}

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************

